Convergence of Adam in Deep ReLU Networks via Directional Complexity and Kakeya Bounds

First-order adaptive optimization methods like Adam are the default choices for training modern deep neural networks. Despite their empirical success, the theoretical understanding of these methods in non-smooth settings, particularly in Deep ReLU networks, remains limited. ReLU activations create exponentially many region boundaries where standard smoothness assumptions break down. \textbf{We derive the first \(\tilde{O}\!\bigl(\sqrt{d_{\mathrm{eff}}/n}\bigr)\) generalization bound for Adam in Deep ReLU networks and the first global-optimal convergence for Adam in the non smooth, non convex relu landscape without a global PL or convexity assumption.} Our analysis is based on stratified Morse theory and novel results in Kakeya sets. We develop a multi-layer refinement framework that progressively tightens bounds on region crossings. We prove that the number of region crossings collapses from exponential to near-linear in the effective dimension. Using a Kakeya based method, we give a tighter generalization bound than PAC-Bayes approaches and showcase convergence using a mild uniform low barrier assumption.

==> sections/001_abstract.tex <==
\begin{abstract}
Adaptive optimizers like Adam and AdamW excel empirically but lack convergence guarantees in non-smooth ReLU networks.
The ReLU-induced piecewise-affine loss has exponentially many polyhedral regions, defying classical analyses.
We prove the first path-wise convergence bounds for Adam and AdamW under mild initialization-margin and diminishing step-size conditions.
Our core is an iterative refinement that leverages margin stability, spectral floor, low-rank drift, and angular concentration to tightly bound activation-pattern changes.
This shrinks region crossings from exponential to near-linear in the effective dimension, yielding convergence rates with only logarithmic depth and parameter dependence.
These results bridge practical performance and theoretical guarantees for deep ReLU models.
\end{abstract}
